Improving Interpretation Faithfulness for Vision Transformers

Vision Transformers (ViTs) have achieved state-of-the-art performance for various vision tasks. One reason behind the success lies in their ability to provide plausible innate explanations for the behavior of neural architectures. However, ViTs suffer from issues with explanation faithfulness, as their focal points are fragile to adversarial attacks and can be easily changed with even slight perturbations on the input image. In this paper, we propose a rigorous approach to mitigate these issues by introducing Faithful ViTs (FViTs). Briefly speaking, an FViT should have the following two properties: (1) The top-$k$ indices of its self-attention vector should remain mostly unchanged under input perturbation, indicating stable explanations; (2) The prediction distribution should be robust to perturbations. To achieve this, we propose a new method called Denoised Diffusion Smoothing (DDS), which adopts randomized smoothing and diffusion-based denoising. We theoretically prove that processing ViTs directly with DDS can turn them into FViTs. We also show that Gaussian noise is nearly optimal for both $\ell_2$ and $\ell_\infty$-norm cases. Finally, we demonstrate the effectiveness of our approach through comprehensive experiments and evaluations. Results show that FViTs are more robust against adversarial attacks while maintaining the explainability of attention, indicating higher faithfulness.

==> tab/abla.tex <==
\begin{table}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc} 
\toprule
\multirow{2}{*}{} & Classification & \multicolumn{2}{c}{Segementation} & \multicolumn{2}{c}{Perturbation Tests}    \\ 
\cmidrule(lr){2-2}\cmidrule(l){3-6}
                  & \textbf{Rob. Acc. (\%)} & \textbf{Rob. Acc. (\%)}  & \textbf{mIOU}            & \textbf{Pos. \textit{P-AUC}} & \textbf{Neg. \textit{P-AUC}}  \\ 
\midrule
\textbf{Ours}              & \textbf{99.5 } & \textbf{ 97.8 } & \textbf{0.985}  & \textbf{ 15.29}     & \textbf{63.23}       \\
\textbf{$-$smoothing}      & 98.2           & 96.3            & 0.977           & 18.51               & 54.65                \\
\textbf{$-$denosing}       & 96.4           & 94.7            & 0.965           & 21.36               & 50.53                \\
\textbf{$-$both}           & 92.1           & 90.5            & 0.947           & 38.13               & 48.58                \\
\bottomrule
\end{tabular}
}
\caption{Results of the ablation study on classification, segmentation, and perturbation tests.}
\label{tab: abl}
\vspace{-12pt}
\end{table}

==> tab/fig4.tex <==
\begin{figure*}[htbp]
\centering
	\subfigure[Pos. Perturbation] %第一张子图
	{
		\begin{minipage}{7cm}
			\centering          %子图居中
    \label{fig:pos-per}
			\includegraphics[scale=0.50]{figs/perturb-auc-pos.pdf} 
		\end{minipage}
	}
	\subfigure[Neg. Perturbation] %第二张子图
	{
		\begin{minipage}{7cm}
			\centering      %子图居中
    \label{fig:pos-neg}
			\includegraphics[scale=0.50]{figs/perturb-auc-neg.pdf}
		\end{minipage}
	}
    \caption{Results of perturbation test. The positive and negative perturbation tests evaluate the importance of pixels for a model's classification by masking out pixels in an input image and measuring the impact on accuracy. For positive perturbation, important pixels are first removed; for negative perturbation, dropping starts from non-related pixels.
    % In positive perturbation, a steep decrease in performance indicates that the masked pixels were important for classification. In negative perturbation, maintaining accuracy while removing pixels unrelated to the class is a sign of good performance.
    }
    \label{fig: per}
\end{figure*}

==> tab/fig5.tex <==
\begin{figure*}[htbp]
\centering
 \subfigure[Sens. w.r.t Diff. Radius] %第三张子图
	{
		\begin{minipage}{7cm}
			\centering      %子图居中
			\label{fig:ver-r}\includegraphics[scale=0.50]{exp/Verify-diff-R.pdf}
		\end{minipage}
	}
 \subfigure[Sens. w.r.t Diff. Sampling Steps] %第四张子图
	{
		\begin{minipage}{7cm}
			\centering      %子图居中
			\label{fig:ver-n}
   \includegraphics[scale=0.50]{exp/Verify-diff-Sample.pdf}
		\end{minipage}
	}
    \caption{Results of verifying faithful region.
    }
    \label{fig: verify}
\end{figure*}

==> tab/fig6.tex <==
\begin{figure*}[!htbp]
\centering
	\subfigure[Pos. Perturbation] %第一张子图
	{
            \label{fig:per-pos}
		\includegraphics[scale=0.33]{figs/perturb-auc-pos.pdf} 
	}
	\subfigure[Neg. Perturbation] %第二张子图
	{
            \label{fig:per-neg}
		\includegraphics[scale=0.33]{figs/perturb-auc-neg.pdf}
	}
     \subfigure[Sens. Diff. Radius] %第三张子图
	{
		\label{fig:ver-r}
            \includegraphics[scale=0.33]{exp/Verify-diff-R.pdf}
	}
    \caption{(a) and (b) are results of the perturbation test. (c) is the sensitivity analysis results.
    %The positive and negative perturbation tests evaluate the importance of pixels for a model's classification by masking out pixels in an input image and measuring the impact on accuracy. For positive perturbation, important pixels are first removed; for negative perturbation, dropping start from non-related pixels.
    % In positive perturbation, a steep decrease in performance indicates that the masked pixels were important for classification. In negative perturbation, maintaining accuracy while removing pixels unrelated to the class is a sign of good performance.
    }
    \label{fig: per}
\end{figure*}

==> tab/tab1.tex <==
\begin{table*}
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{
Robustness comparison.
}
\label{golden}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{cccccccccccc} 
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perturbation\\Radius\end{tabular}} & \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{ImageNet}                        & \multicolumn{3}{c}{Cityscape}                       & \multicolumn{3}{c}{COCO}                             \\ 
\cmidrule(l){4-12}
                                                                              &                        &                         & Clean             & Corrupt        & Reten.         & Clean             & Corrupt        & Reten.         & Clean             & Corrupt        & Reten.          \\ 
\midrule
\multirow{12}{*}{$\delta=0.1$}                                                & \multirow{4}{*}{VIT}   & Vanilla-AT              & 0.002             & 20.145         & 0.663          & 0.019             & 19.566         & 0.811          & 0.009             & 15.576         & 0.553           \\
                                                                              &                        & Rollout               & 0.028             & 1.824          & 0.627          & 0.016             & 1.130          & 0.798          & 0.026             & 1.170          & 0.527           \\
                                                                              &                        & GradCAM               & 0.042             & 2.691          & 0.653          & 0.023             & 1.277          & \textbf{0.815} & 0.022             & 1.049          & 0.523           \\
                                                                              &                        & Ours                    & \textbf{3.81E-08} & \textbf{1.750} & \textbf{0.672} & \textbf{2.75E-07} & \textbf{1.099} & 0.813          & \textbf{1.79E-09} & \textbf{0.908} & \textbf{0.579}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{DeiT}  & Vanilla                 & 0.002             & 23.447         & 0.612          & 0.027             & 18.640         & \textbf{0.809} & 0.060             & 15.633         & 0.524           \\
                                                                              &                        & Rollout               & 0.050             & 1.927          & 0.662          & 0.020             & 0.810          & 0.798          & 0.084             & 1.537          & 0.538           \\
                                                                              &                        & GradCAM               & 0.058             & 1.139          & 0.640          & 0.034             & 1.037          & 0.802          & 0.091             & 1.590          & 0.530           \\
                                                                              &                        & Ours                    & \textbf{1.23E-08} & \textbf{0.736} & 0.670          & \textbf{1.80E-08} & \textbf{0.777} & 0.802          & \textbf{8.49E-09} & \textbf{1.030} & \textbf{0.543}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{Swin}  & Vanilla                 & 0.024             & 2.127          & \textbf{0.721} & 0.005             & 2.605          & 0.912          & 0.036             & 1.771          & 0.493           \\
                                                                              &                        & Rollout               & 0.085             & 0.060          & 0.694          & 0.267             & 0.055          & 0.900          & 0.170             & 0.043          & \textbf{0.554}  \\
                                                                              &                        & GradCAM               & 0.584             & 0.029          & 0.694          & 0.241             & 0.054          & 0.895          & 0.166             & 0.049          & 0.496           \\
                                                                              &                        & Ours                    & \textbf{4.70E-07} & \textbf{0.002} & 0.713          & \textbf{2.77E-07} & \textbf{0.036} & 0.907          & \textbf{2.42E-06} & \textbf{0.042} & 0.45            \\
                                                    
\midrule
\multirow{12}{*}{$\delta=0.2$}                                                & \multirow{4}{*}{VIT}   & Vanilla-AT              & 0.002             & 20.145         & 0.663          & 0.019             & 19.566         & 0.811          & 0.009             & 15.576         & 0.553           \\
                                                                              &                        & Rollout               & 0.028             & 1.824          & 0.627          & 0.016             & 1.130          & 0.798          & 0.026             & 1.170          & 0.527           \\
                                                                              &                        & GradCAM               & 0.042             & 2.691          & 0.653          & 0.023             & 1.277          & \textbf{0.815} & 0.022             & 1.049          & 0.523           \\
                                                                              &                        & Ours                    & \textbf{3.81E-08} & \textbf{1.750} & \textbf{0.672} & \textbf{2.75E-07} & \textbf{1.099} & 0.813          & \textbf{1.79E-09} & \textbf{0.908} & \textbf{0.579}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{DeiT}  & Vanilla                 & 0.002             & 23.447         & 0.612          & 0.027             & 18.640         & \textbf{0.809} & 0.060             & 15.633         & 0.524           \\
                                                                              &                        & Rollout               & 0.050             & 1.927          & 0.662          & 0.020             & 0.810          & 0.798          & 0.084             & 1.537          & 0.538           \\
                                                                              &                        & GradCAM               & 0.058             & 1.139          & 0.640          & 0.034             & 1.037          & 0.802          & 0.091             & 1.590          & 0.530           \\
                                                                              &                        & Ours                    & \textbf{1.23E-08} & \textbf{0.736} & 0.670          & \textbf{1.80E-08} & \textbf{0.777} & 0.802          & \textbf{8.49E-09} & \textbf{1.030} & \textbf{0.543}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{Swin}  & Vanilla                 & 0.024             & 2.127          & \textbf{0.721} & 0.005             & 2.605          & 0.912          & 0.036             & 1.771          & 0.493           \\
                                                                              &                        & Rollout               & 0.085             & 0.060          & 0.694          & 0.267             & 0.055          & 0.900          & 0.170             & 0.043          & \textbf{0.554}  \\
                                                                              &                        & GradCAM               & 0.584             & 0.029          & 0.694          & 0.241             & 0.054          & 0.895          & 0.166             & 0.049          & 0.496           \\
                                                                              &                        & Ours                    & \textbf{4.70E-07} & \textbf{0.002} & 0.713          & \textbf{2.77E-07} & \textbf{0.036} & 0.907          & \textbf{2.42E-06} & \textbf{0.042} & 0.45            \\
                                                            
\midrule
\multirow{12}{*}{$\delta=0.3$}                                                & \multirow{4}{*}{VIT}   & Vanilla-AT              & 0.002             & 20.145         & 0.663          & 0.019             & 19.566         & 0.811          & 0.009             & 15.576         & 0.553           \\
                                                                              &                        & Rollout               & 0.028             & 1.824          & 0.627          & 0.016             & 1.130          & 0.798          & 0.026             & 1.170          & 0.527           \\
                                                                              &                        & GradCAM               & 0.042             & 2.691          & 0.653          & 0.023             & 1.277          & \textbf{0.815} & 0.022             & 1.049          & 0.523           \\
                                                                              &                        & Ours                    & \textbf{3.81E-08} & \textbf{1.750} & \textbf{0.672} & \textbf{2.75E-07} & \textbf{1.099} & 0.813          & \textbf{1.79E-09} & \textbf{0.908} & \textbf{0.579}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{DeiT}  & Vanilla                 & 0.002             & 23.447         & 0.612          & 0.027             & 18.640         & \textbf{0.809} & 0.060             & 15.633         & 0.524           \\
                                                                              &                        & Rollout               & 0.050             & 1.927          & 0.662          & 0.020             & 0.810          & 0.798          & 0.084             & 1.537          & 0.538           \\
                                                                              &                        & GradCAM               & 0.058             & 1.139          & 0.640          & 0.034             & 1.037          & 0.802          & 0.091             & 1.590          & 0.530           \\
                                                                              &                        & Ours                    & \textbf{1.23E-08} & \textbf{0.736} & 0.670          & \textbf{1.80E-08} & \textbf{0.777} & 0.802          & \textbf{8.49E-09} & \textbf{1.030} & \textbf{0.543}  \\ 
\cmidrule{2-12}
                                                                              & \multirow{4}{*}{Swin}  & Vanilla                 & 0.024             & 2.127          & \textbf{0.721} & 0.005             & 2.605          & 0.912          & 0.036             & 1.771          & 0.493           \\
                                                                              &                        & Rollout               & 0.085             & 0.060          & 0.694          & 0.267             & 0.055          & 0.900          & 0.170             & 0.043          & \textbf{0.554}  \\
                                                                              &                        & GradCAM               & 0.584             & 0.029          & 0.694          & 0.241             & 0.054          & 0.895          & 0.166             & 0.049          & 0.496           \\
                                                                              &                        & Ours                    & \textbf{4.70E-07} & \textbf{0.002} & 0.713          & \textbf{2.77E-07} & \textbf{0.036} & 0.907          & \textbf{2.42E-06} & \textbf{0.042} & 0.45            \\
\bottomrule
\end{tabular}
}
% \caption{The main results}
\end{table*}
